BeamScatter: Scalable, Deployable Long-Range backscatter communication with Beam-Steering

WiFi backscatter tags can enable direct connectivity of IoT devices with commodity WiFi hardware at low power. However, most state of the art backscatter tag implementations in this area have limited transmitter to tag range, are not suitable to be deployed in a WiFi mesh network, and do not take full advantage of today's WiFi network capabilities such as MIMO. In this paper, we present BeamScatter, which can realize a backscatter tag based on MIMO techniques that can work at a very long separation of 28m from an access-point and enables their deployment in WiFi mesh networks. BeamScatter presents a novel technique to perform beam-steering on the MIMO tag at a very low power consumption of 88 uW while achieving a peak throughput of 500kbps. Next, BeamScatter creates a novel modeling framework to decide the optimal phase setting on the tag to steer the backscattered signal WiFi access point.

==> Makefile <==
TARGET           ?= paper
TARGET_TYPE      ?= pdf
LATEXMK          ?= latexmk
LATEXDIFF        ?= latexdiff-vc

ifneq ($(V), 1)
Q                := @
LATEXMK_FLAGS    += -silent
else
Q                :=
LATEXDIFF_FLAGS  += -V
endif

UNAME_S          := $(shell uname -s)
TARGET_FILE       = $(TARGET).$(TARGET_TYPE)
TARGET_DIFF       = $(TARGET)-diff$(LATEXDIFF_BASE)

LATEXMK_FLAGS    += -$(TARGET_TYPE) -f

# Reference git branch/tag
LATEXDIFF_BASE   := submission2
LATEXDIFF_STYLE  := TRADITIONAL
# NOTE: vc-version does not take preamble
LATEXDIFF_FLAGS  += --git --flatten --force -r $(LATEXDIFF_BASE) 
LATEXDIFF_IGNORE := author,authornote,email,affiliation,institution,ccsdesc,renewcommand,section,subsecion,subsubsection
LATEXDIFF_NOENV  := (?:picture|DIFnomarkup|align|comment|CCSXML|thebibliography|figure|equation|tabular)[\w\d*@]*
LATEXDIFF_FLAGS  += --exclude-textcmd='$(LATEXDIFF_IGNORE)'

ifeq ($(shell which $(LATEXMK)), )
$(error "Please install `$(LATEXMK)`!")
endif
ifeq ($(shell which $(LATEXDIFF)), )
$(warning "Please install `latexdiff` or `latexdiff-vc` to use `make diff` function!")
endif

.PHONY: clean view check diff

$(TARGET_FILE): $(wildcard *.tex *.bib *.sty *.cls figures/*)
	@echo "Compiling..."
	$(Q) $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET)

clean:
	@echo "Cleaning..."
	$(Q) $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET) -C
	$(Q) rm -f $(TARGET).bbl $(TARGET_DIFF).bbl
	$(Q) if test -f $(TARGET_DIFF).tex; then $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET_DIFF) -C; rm $(TARGET_DIFF).tex; fi

view: $(TARGET_FILE)
ifeq ($(OS), Windows_NT)
	$(Q) open $(TARGET_FILE)
else
ifeq ($(UNAME_S), Linux)
	$(Q) xdg-open $(TARGET_FILE) &
endif
ifeq ($(UNAME_S), Darwin)
	$(Q) open $(TARGET_FILE) &
endif
endif

check: $(TARGET_FILE)
	$(Q) grep -i -e "undefined" -e "multiply" $(TARGET).log || echo "Nothing found."

# NOTE: latexdiff will not work with IEEEtran style
diff: clean
	@echo "Compiling diff..."
	$(Q) $(LATEXDIFF) $(LATEXDIFF_FLAGS) $(TARGET).tex
	$(Q) $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET_DIFF)


==> evaluation.tex <==
% !TEX root = main.tex


% \begin{figure*}[t]
%  \centering
%  \begin{minipage}{\textwidth}
%   \includegraphics[width=\linewidth]{figures/Fig_Beam_pattern_V1-crop.pdf}
% \caption{\textbf{(a)} CLC-based $\pi$ matching network, \textbf{(b)} Schematic of passive pseudo-balun ED,\textbf{(c)} Schematic of LNA, \textbf{(d)} Transmission-line-less SSB QPSK Backscatter.}
%  \label{fig:backscatter}
%  \end{minipage}
% \end{figure*}



 \begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/Fig_Beam_pattern_V1-crop.pdf}
    \caption{Beampatterns of the measured backscatter signal for different phase settings($\Delta$ denotes the phase difference between the consecutive antennas) when the excitation signal is incident normal to the tag . The measured beampatterns are compared to the theoretical beampatterns. The measured beam-steering angles match very closely to that of the theoretical value.}
    \label{fig:beampatterns}
\end{figure*}

\section{Evaluation}
In this section, we will present preliminary results demonstrating the working of the \name's beam-steering tag and the advantages offered by it compared to the traditional single antenna backscatter tags. We will also show the effectiveness of the proposed algorithm in determining the best phase configuration on the tag. 

 \begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/Fig_Distance_Compare_V1-crop.pdf}
    \caption{Comparison of feasible Transmitter to Tag and Tag to Receiver separations for SyncScatter tag\cite{dunna2021syncscatter}, Retro-reflective tag\cite{meng202112} and the proposed \name tag.}
    \label{fig:D1_D2_plot}
\end{figure}

\subsection{Beampattern Measurement:}
 Here we present a micro-benchmark to demonstrate beam-steering ability by measuring the beam-pattern of the backscattered signals. For this measurement, we place a WiFi transmitter and the \name tag such that the signal from the transmitter is incident normally on the tag. Then we move the receiver around the tag in a circle by maintaining constant distance between the Tag and the WiFi receiver and record the received power at every point on the circle. We repeat this method for different tag configurations(different $\Delta$- phase shift between consecutive antennas) and plot the received signal power as a function of the receiver rotation angle to obtain the measured beam-patterns. Finally, we compare the measured beam-patterns with the theoretical beam-pattern as shown in Fig~\ref{fig:beampatterns}. The measured beam-patterns closely resemble that of the patterns dictated by the theory in all the cases.
\subsection{Finding tag's Best configuration:}
 Here we present the simulation results of our proposed algorithm to find the best phase configuration on the tag that results in maximizing the backscattered signal power at the receiver. For this, we simulate by placing the WiFi transmitter AP 10m away from the tag and the receiver at arbitrary locations and obtain the wireless channel from the transmitter to the receiver via the tag. We also note the ground truth angular location of the transmitter and the receiver with reference to the normal of the backscatter tag and compute the phase shifts that are needed to be given at each antenna on the tag to achieve constructive combination of the backscattered signal at the receiver. Then using the simulated wireless channel, we estimate the parameter $\alpha = \frac{2\pi}{\lambda}d(sin(\theta_1) + sin(\theta_2))$ using the algorithm outlined in section 3 and compare the estimates with the ground truth. Fig~\ref{fig:alpha_estimate1} plots the CDF of the estimated value of alpha by placing the Rx WiFi AP along $\theta=0$ degree for different Rx to Tag separations(denoted by $r$). Similarly, Fig~\ref{fig:alpha_estimate2} plots the CDF by placing the Rx WiFi AP along $\theta = 60$ from the normal. We observe that the estimates of alpha are very reliable when the Rx is close to the tag. As the Rx separation from the tag increases, the CDF curve becomes broader indicating that the estimates are less reliable due to the decrease in SNR in the channel measurements. Even at larger Rx to tag separation of 30m, the algorithm works accurately in 80\% of the cases.    
 

\begin{figure}[h]
\centering
\begin{minipage}{0.23\textwidth}
\includegraphics[width=\linewidth]{figures/alpha_est1-crop.pdf}
\subcaption{Receiver AP at theta = 0 degrees}
\label{fig:alpha_estimate1}
\end{minipage}
\begin{minipage}{0.23\textwidth}
\includegraphics[width=\linewidth]{figures/alpha_est2-crop.pdf}
\subcaption{Receiver AP at theta = 60 degrees}
\label{fig:alpha_estimate2}
\end{minipage}
%\vspace{-0.2in}
\caption{Figure showing the CDF of the estimated parameter alpha values when receiver AP is placed at different distances from the tag for the case of normal incidence.}
%\vspace{-0.15in}
\end{figure}

\subsection{Range Improvement:}
Here we show the improvement in the tag deployment range offered by the \name's beam-steering tag and compare it with the previous approaches in \cite{ISSCC-backscatter,hitchhike}. The improvement is shown in terms of comparing the possible Tx to Tag and Tag to Rx separations for the \name's backscatter tag with other backscatter tag implementations. Fig~\ref{fig:D1_D2_plot} plots the feasible separations for the tag from the Tx and the Rx to establish a backscatter link. As can be seen in Fig~\ref{fig:D1_D2_plot}, the previous works SyncScatter\cite{dunna2021syncscatter} has a maximum separation of 15 m from both the Tx and Rx WiFi APs and Retro-reflective MIMO\cite{meng202112} implementation has maximum separation of 23m from the co-located AP with Tx and Rx. On the other hand, \name tag can support upto 28 m separation from either of the APs thus supporting mesh networks with >50m AP to AP separation.  











==> feasibility-mani.tex <==
% !TEX root = main.tex
\section{Background and Motivation}
WiFi backscatter communication provides a useful way to convey information by piggybacking\cite{interscatter,hitchhike,passive-wifi} on the existing RF signals in the environment instead of generating the RF signals locally. This way of communicating enables us to deploy low power battery assisted devices that can have a very long life up to a few years. In the paradigm of backscatter communication, a transmitter sends signals which acts as an excitation signal to the backscatter tag.The backscatter tag embeds its data by modulating the excitation signal which is used by the receiver to decode the tag data. By equipping a device with a backscatter tag, for instance an IoT device\cite{blink}, it can be provided internet connectivity at a very low energy footprint. 

For easy and large-scale adaptation of backscatter tags, the backscatter tags have to be compatible with widely available existing infrastructure like WiFi access points. Also, the excitation signals should be used for productive communication i.e. backscatter tags should not limit the excitation signals to be used for just conveying tag data. Hitchhike\cite{hitchhike} presents a way of communicating with backscatter tags using COTS WiFi devices by modulating the excitation WiFi packets on one channel to a non-overlapping WiFi channel. But it has a limitation that the backscatter tag should be placed very close to the transmitting WiFi AP. The issue of placing the tag close to the transmitter is due to the lack of Synchronization at the backscatter tags.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/Fig2_V1-crop.pdf}
    \caption{Figure showing the backscattered signal spectrum and the transmit signal leakage when the transmitter and receiver are co-located. The transmit leakage dominates the backscattered signal power beyond a certain AP to tag separation and limits the range for the retro-reflective backscatter tag.}
    \label{fig:spectrum-mask}
\end{figure}

SyncScatter\cite{dunna2021syncscatter} resolves the transmitter to tag placement issue by introducing the idea of a hierarchical wake-up receiver. But even with synchronization, the backscatter tags have a limited maximum range of 13 m from a Wireless access point and still remain a barrier to realize the tag deployment in a WiFi mesh network where access-points are separated by ~50m from one another. 

\textbf{Van-atta based solution}: To address the limited range problem, a simple idea used in the prior work\cite{meng202112} is to enable MIMO with van-atta structure\cite{sharp1960van} to extend the range of a backscatter tag from a WiFi access point to 23m. The idea here is that the backscatter tags are made retro-reflective by placing multiple antennas on them. The multiple antennas on the tag result in additional array gain compared to single antenna tags and increase the backscattered signal power from the tag. The increased backscattered power translates to supporting a backscatter link for a larger Tx to tag separation than single antenna tags. But the idea of using retro-reflective tags meant that the Transmitter and the Receiver WiFi AP are co-located with each other which introduce more implementation challenges. 

The primary challenge is that, a co-located Tx and Rx means there will be a lot of self interference\cite{self-interference} from the transmitter to the receiver. To understand this, consider the spectrum mask\cite{spec_mask} for the WiFi standard as shown in Fig~\ref{fig:spectrum-mask}. The backscattered signal from the tag is also shown here for comparison. As we can see, the signal leakage from the transmitter is far higher than the backscattered signal at the receiver AP and causes a series of problems in the RF front-end processing. Although the transmitter leakage and backscattered signal are on two different channels, commercial WiFi access points do not have a very strong analog filter to remove the leakage signal. Hence, the strong transmitter leakage signal acts as a Jammer to the backscattered signal and causes gain compression at the amplifier in the RF-front end. This non-linearity results in a signal occupying the same frequency band as the backscattered signal and is much stronger than backscattered signal leading to poor decoding of backscattered signal from the tag. 

\textbf{Proposed solution: }To address the issues with co-located Tx and Rx, we propose a new tag design that takes advantage of the multiple antennas on the tag to support large Tx to tag range while simultaneously eliminating the self-interference problem. Our idea here is to modify the tag design such that the backscatter tag can steer the incident signals towards a different AP as shown in Fig~\ref{fig:intro} rather than towards the same transmitting AP. Steering the backscattered signal towards a different AP solves the self-interference problem and will not cause any non-linear effects\cite{non_linearity} at the receiver. In the next section, we explain how we can design such a tag that can steer the backscattered signal.    
% \begin{itemize}
%     \item Excitation signal should be productive communication with existing COTS WiFi communication. 
%     \item The excitation should not interfere with the reception or hurt the dynamic range of the reception.
%     \item 
% \end{itemize}






==> feasibility.tex <==
% !TEX root = main.tex
\section{Background and Motivation}

Ideal Requirements from backscatter communication systems. 

\begin{itemize}
    \item Excitation signal should be productive communication with existing COTS WiFi communication. 
    \item The excitation should not interfere with the reception or hurt the dynamic range of the reception.
    \item 
\end{itemize}


\textbf{Van-atta based solution}: A simple idea used in some prior work is to enable MIMO with van-atta structure, this makes it challenging. For example, imagine the excitation radio transmitting the signals  challenge with the back-scatter. 

